Local 3D Editing via 3D Distillation of CLIP Knowledge

3D content manipulation is an important computer vision task with many real-world applications (e.g., product design, cartoon generation, and 3D Avatar editing). Recently proposed 3D GANs can generate diverse photorealistic 3D-aware contents using Neural Radiance fields (NeRF). However, manipulation of NeRF still remains a challenging problem since the visual quality tends to degrade after manipulation and suboptimal control handles such as 2D semantic maps are used for manipulations. While text-guided manipulations have shown potential in 3D editing, such approaches often lack locality. To overcome these problems, we propose Local Editing NeRF (LENeRF), which only requires text inputs for fine-grained and localized manipulation. Specifically, we present three add-on modules of LENeRF, the Latent Residual Mapper, the Attention Field Network, and the Deformation Network, which are jointly used for local manipulations of 3D features by estimating a 3D attention field. The 3D attention field is learned in an unsupervised way, by distilling the zero-shot mask generation capability of CLIP to the 3D space with multi-view guidance. We conduct diverse experiments and thorough evaluations both quantitatively and qualitatively.

==> Tables/Table_MSE.tex <==
\begin{table}[t!]
\begin{center}
\caption{Table caption}
\label{table_MSE}
\footnotesize
\begin{tabular}[\linewidth]{l | cccccccc}
\toprule
Method & Elf ear & \makecell{Open\\mouth} & Big lips & Smiling & Surprised & ??? & ... & Avg. \\
\midrule
FeNeRF + StyleGAN &
0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 && 0.00 \\
LeNeRF w/o AFN &
0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 && 0.00 \\
\textbf{LeNeRF (Ours)} &
0.00 & 0.00 & 0.00 & 0.00 & 0.00 & 0.00 && 0.00 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}


==> Tables/Table_Test.tex <==
\begin{table}[t!]
\begin{center}
\caption{Table caption}
\label{table_test}
\begin{tabular}[\linewidth]{l | ccc}
\toprule
Test & 0.00 & 0.00 & 0.00 \\
\midrule
Test & 0.00 & 0.00 & 0.00 \\
\bottomrule
\end{tabular}
\end{center}
\end{table}
